Hydra: Hybrid Server Power Model

With the growing complexity of big data workloads that require abundant data and computation, data centers consume a tremendous amount of power daily. In an effort to minimize data center power consumption, several studies developed power models that can be used for job scheduling either reducing the number of active servers or balancing workloads across servers at their peak energy efficiency points. Due to increasing software and hardware heterogeneity, we observed that there is no single power model that works the best for all server conditions. Some complicated machine learning models themselves incur performance and power overheads and hence it is not desirable to use them frequently. There are no power models that consider containerized workload execution. In this paper, we propose a hybrid server power model, Hydra, that considers both prediction accuracy and performance overhead. Hydra dynamically chooses the best power model for the given server conditions. Compared with state-of-the-art solutions, Hydra outperforms across all compute-intensity levels on heterogeneous servers.

==> container_model.tex <==
\usepackage{tikz}
\pagestyle{empty}

\def\layersep{2.5cm}

\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=17pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron, fill=green!50];
    \tikzstyle{output neuron}=[neuron, fill=red!50];
    \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
    \tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,4}
    % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
        \node[input neuron, pin=left:Input \#\y] (I-\name) at (0,-\y) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,5}
        \path[yshift=0.5cm]
            node[hidden neuron] (H-\name) at (\layersep,-\y cm) {};

    % Draw the output layer node
    \node[output neuron,pin={[pin edge={->}]right:Output}, right of=H-3] (O) {};

    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,5}
            \path (I-\source) edge (H-\dest);

    % Connect every node in the hidden layer with the output layer
    \foreach \source in {1,...,5}
        \path (H-\source) edge (O);

    % Annotate the layers
    \node[annot,above of=H-1, node distance=1cm] (hl) {Hidden layer};
    \node[annot,left of=hl] {Input layer};
    \node[annot,right of=hl] {Output layer};
\end{tikzpicture}
% End of code


==> usecase.tex <==

\section{Use Case : DNN-Accelerated Load Migration for Energy-efficient Data Center}

\subsection{Dockerized Application Migration}
The various applications are run on the workload servers as necessary. New applications may be started and running applications will be shut down as needed. A standalone server has the DNN and RNN power prediction model running on it, which triggers the migration on each of the application servers (represented as GPU server in Fig.~\ref{fig.integrated_sys_design}).
The system parameters are fed from these servers to Power Prediction Model. These parameters are used to predict the power values. If the predicted power is greater than the configured optimal value for the server, then the server workload is migrated to another server which has lower power utilization.
The integrated system design is seen in Fig. 5, where multiple servers concurrently feed their system parameters to the Power Prediction Model.
\begin{figure}
\centering
\includegraphics[width=9cm]{./fig/Integrated System Design.png}
\caption{Integrated System Design} \label{fig.integrated_sys_design}
\end{figure}


We ran applications with the widely used virtualization system, Docker~\cite{docker}. Containers in Docker are isolated from each other and bundle their own tools, libraries and configuration files; they can communicate with each other through well-defined channels. We ran individual applications in a separate containers and migrated the applications between servers in container level. This way, we do not need to worry about  dependency and compatibility issues on different servers. 
We used Checkpoint Restore in User Space (CRIU) for creating checksums of migrating applications. CRIU creates custom checkpoint, saves the process state and stops the container. This process state can be transferred to another server and the container can be restored with the same process state which is being transferred. Once a migration is determined, four steps of migration are processed; 1) Docker commit (saves the running container’s file system), 2) Docker save (saves the container file system into a compressed file), 3) transfer the compressed image to another server, and 4) loads the file into a Docker image and run a container.


%We evaluated our load migration algorithm on a cluster of three servers as shown in Figure 2. All three servers are connected through SJSU network. The GPU server is a coordinator and a stress-feed server for the other two worker servers. The GPU server runs the load migration agent which is fed with system statistics from the two worker servers periodically. The DNN-based power model is accelerated with the GPU on the GPU server. Once the power model estimates that one of the server exceeds the peak efficiency point, the migration is commanded based on the algorithm in Algorithm 1. Two worker servers run CloudSuite applications (media streaming, web server and web search) and serve the data center operations. Each of the worker servers has a 32-core Intel Xeon processor and a 128GB memory. Both servers run CentOS v7. To enable Docker-based migration, we used Docker swarm which generates two random tokens, a worker token and a manager token. GPU server uses manager token and the other two worker servers used worker tokens such that the migration is commanded by the GPU server through the Docker swarm. 

\subsection{Migration Optimization}
